Implications of Poincare symmetry for thermal field theories in finite-volume

The analytic continuation to an imaginary velocity $i\xi$ of the canonical partition function of a thermal system expressed in a moving frame has a natural implementation in the Euclidean path-integral formulation in terms of shifted boundary conditions. Writing the Boltzmann factor as $\exp[-L_0(H-i\xi.P)]$, the Poincare invariance underlying a relativistic theory implies a dependence of the free-energy on $L_0$ and the shift $\xi$ only through the combination $\beta= L_0 \sqrt{1+\xi^2}$. This in turn implies a set of Ward identities, some of which were previously derived by us, among the correlators of the energy-momentum tensor. In the infinite-volume limit they lead to relations among the cumulants of the total energy distribution and those of the momentum, i.e. they connect the energy and the momentum distributions in the canonical ensemble. In finite volume the Poincare symmetry translates into exact relations among partition functions and correlation functions defined with different sets of (generalized) periodic boundary conditions. They have interesting applications in lattice field theory. In particular, they offer Ward identities to renormalize non-perturbatively the energy-momentum tensor and novel ways to compute thermodynamic potentials. At fixed bare parameters they also provide a simple method to vary the temperature in much smaller steps than with the standard procedure.

==> dlogZdVmunu.tex <==

\section{Derivation of \eq(\ref{eq:dlogZdVmn}) \la{sec:dlogZ}}

Here we prove the equation (\ref{eq:dlogZdVmn}),
\be % \la{eq:dlogZdVmn}
\frac{\partial\log Z(V)}{\partial V_{\mu\nu}} = \<T_{\mu\nu}\> \cdot {\rm det}_{\nu}(V),
\ee
where ${\rm det}_\nu(V)$ is the determinant of the  $\nu^{\rm th}$ principal minor of the
matrix $V$ (i.e.\ the determinant of the $(d-1)\times(d-1)$ matrix
obtained by removing the $\nu^{\rm th}$ column and $\nu^{\rm th}$ row
from $V$).  As an example, if $V={\rm diag}(L_0,L_1,L_2,L_3)$,
$\partial\log Z/\partial L_\mu = \<T_{\mu\mu}\>
\prod_{\nu\neq\mu}L_\nu$ (no summation over $\mu$ implied).

When $\nu=0$, the statement (\ref{eq:dlogZdVmn}) follows from
the canonical definition of the partition function,
\be
Z(V) = \tr\{e^{-V_{00}\widehat H + i V_{\underline{k}0} \widehat P_{\underline k}}\} 
\ee
and the relations 
\be
\<\!\<\widehat H\>\!\> = - {\rm det}_0(V)\; \<T_{00}\>,
\qquad \qquad 
\<\!\<\widehat P_k\>\!\> = -i\, {\rm det}_0(V)\; \<T_{k0}\>.
\ee
The principal minor ${\rm det}_0(V)$ yields the spatial volume of the system.

For $\nu\neq 0$, we can demonstrate \eq(\ref{eq:dlogZdVmn}) as
follows.  We conjugate $V$ by an even permutation $V'=\Pi^{-1} V \Pi$,
to bring the $\nu^{\rm th}$ column into the first column. Secondly
\eq(\ref{eq:dlogZdVmn}) is used on $Z(V')$ for $\nu=0$, and then
interpreted in terms of $V$ by performing the inverse permutation.

A corollary of \eq(\ref{eq:dlogZdVmn}) is that 
\be 
{\rm det}_\mu(V)
\frac{\partial\log Z(V)}{\partial V_{\mu\nu}}  
=
{\rm det}_\nu(V)
\frac{\partial\log Z(V)}{\partial V_{\nu\mu}},
\qquad \textrm{(no summation implied)}
\ee
since we can choose the energy-momentum tensor to be symmetric.

